WaveCert: Translation Validation for Asynchronous Dataflow Programs via Dynamic Fractional Permissions

Coarse-grained reconfigurable arrays (CGRAs) have gained attention in recent years due to their promising power efficiency compared to traditional von Neumann architectures. To program these architectures using ordinary languages such as C, a dataflow compiler must transform the original sequential, imperative program into an equivalent dataflow graph, composed of dataflow operators running in parallel. This transformation is challenging since the asynchronous nature of dataflow graphs allows out-of-order execution of operators, leading to behaviors not present in the original imperative programs. We address this challenge by developing a translation validation technique for dataflow compilers to ensure that the dataflow program has the same behavior as the original imperative program on all possible inputs and schedules of execution. We apply this method to a state-of-the-art dataflow compiler targeting the RipTide CGRA architecture. Our tool uncovers 8 compiler bugs where the compiler outputs incorrect dataflow graphs, including a data race that is otherwise hard to discover via testing. After repairing these bugs, our tool verifies the correct compilation of all programs in the RipTide benchmark suite.

==> Makefile <==
# LaTeX Makefile
#   Version: 0.4.0
#   Author: Jay Bosamiya <jaybosamiya AT gmail DOT com>
#
# Always find the latest version at
#    https://github.com/jaybosamiya/latex-paper-template/
#
# Alternatively, run `make update-makefile` to pull the latest
# version.

#   ____             __ _                       _   _
#  / ___|___  _ __  / _(_) __ _ _   _ _ __ __ _| |_(_) ___  _ __
# | |   / _ \| '_ \| |_| |/ _` | | | | '__/ _` | __| |/ _ \| '_ \
# | |__| (_) | | | |  _| | (_| | |_| | | | (_| | |_| | (_) | | | |
#  \____\___/|_| |_|_| |_|\__, |\__,_|_|  \__,_|\__|_|\___/|_| |_|
#                         |___/

# If set to 't', all .tex files in the current directory should be
# compiled over to .pdf files.
ALL_FILES_MODE?=

# If set then MAIN_TARGET is used as the root tex file of the project
# to be built.
MAIN_TARGET?=

# If set to git commits, separated by spaces, then `make diff` will
# produce diffs against each commit. Additionally, `make diff-REV`
# will produce a diff against revision REV. Requires `latexdiff` to be
# installed on the system.
#
# Caveat: Works only in MAIN_TARGET mode (for now).
DIFF_REVISIONS?=

# If set to a non-empty value, generates a nice HTML copy of the
# PDF. Requires pdf2htmlex to be installed.
HTML_GENERATION?=

# If set to 't', ensures indentation of all the .tex files is
# normalized using the ./.latexindent.yaml settings.
ALWAYS_REINDENT?=t

################## DON'T CHANGE ANYTHING BEYOND THIS LINE ####################

#     _         _                        _   _        ____        _
#    / \  _   _| |_ ___  _ __ ___   __ _| |_(_) ___  |  _ \ _   _| | ___  ___
#   / _ \| | | | __/ _ \| '_ ` _ \ / _` | __| |/ __| | |_) | | | | |/ _ \/ __|
#  / ___ \ |_| | || (_) | | | | | | (_| | |_| | (__  |  _ <| |_| | |  __/\__ \
# /_/   \_\__,_|\__\___/|_| |_| |_|\__,_|\__|_|\___| |_| \_\\__,_|_|\___||___/
#

.PHONY: all
TEXFILES:=$(wildcard *.tex)

AUTOPICK:=main.tex paper.tex writeup.tex

ALL_TARGET:=

ifeq ($(ALWAYS_REINDENT), t)
all: indent
endif

ifeq ($(ALL_FILES_MODE), t)
ifneq ($(MAIN_TARGET),)
all:
	@echo "Both ALL_FILES_MODE and MAIN_TARGET are set."
	@echo ""
	@echo "Do you mean to compile all of them individually to PDFs?"
	@echo "  If so, please change over to ALL_FILES_MODE"
	@echo ""
	@echo "Do you mean to compile it to a single PDF?"
	@echo "  If so, please set MAIN_TARGET"
	@echo ""
	@echo "Quitting."
else
ALL_TARGET:=$(TEXFILES:.tex=.pdf)
endif
# End of ALL_FILES_MODE
else ifneq ($(MAIN_TARGET),)
ALL_TARGET:=$(MAIN_TARGET:.tex=).pdf
# End of MAIN_TARGET
else
all:
ifeq ($(words $(TEXFILES)), 1)
ALL_TARGET:=$(TEXFILES:.tex=.pdf)
else ifeq ($(words $(filter $(AUTOPICK),$(TEXFILES))), 0)
all:
	@echo "Found $(words $(TEXFILES)) .tex files."
	@echo ""
ifeq ($(words $(TEXFILES)), 0)
else
	@echo "Do you mean to compile all of them individually to PDFs?"
	@echo "  If so, please change over to ALL_FILES_MODE"
	@echo ""
	@echo "Do you mean to compile it to a single PDF?"
	@echo "  If so, please set MAIN_TARGET"
	@echo ""
endif
	@echo "Quitting."
else
AUTOROOTCHOICE:=$(firstword $(foreach V,$(AUTOPICK),$(filter $(V),$(TEXFILES))))
all: $(warning Found multiple .tex files. Automatically chosing likely root as $(AUTOROOTCHOICE). Set either MAIN_TARGET or ALL_FILES_MODE to squash this warning.) $(AUTOROOTCHOICE:.tex=.pdf)
endif
endif

ifneq ($(ALL_TARGET),)
ifeq ($(HTML_GENERATION),)
all: $(ALL_TARGET)
else
all: $(ALL_TARGET:.pdf=.html)
endif
endif

LATEXRUN:=python3 ./.latexrun --latex-args='--synctex=1' -O .latex.out
# Note: We use latexrun from a slightly more up-to-date fork available
# at https://github.com/Nadrieril/latexrun
# The original can be found at https://github.com/aclements/latexrun

# Use the correct sed necessary, based upon OS
UNAME_S:=$(shell uname -s)
ifeq ($(UNAME_S),Linux)
SED:=sed
else
ifeq ($(UNAME_S),Darwin)
SED:=gsed
else
$(error Unrecognized OS "$(UNAME_S)" when trying to autodetect sed)
endif
endif

.PHONY: FORCE
%.pdf: FORCE ./.latexrun
	@$(LATEXRUN) $*.tex
	@cp .latex.out/*.synctex.gz .
	@echo "Finished building $@"

%.html: %.pdf
	@echo "Generating $@"
	@pdf2htmlEX --zoom 2 --process-outline 0 $<

.PHONY: clean
clean: ./.latexrun
	@$(LATEXRUN) --clean-all
	@rm -rf *.synctex.gz ./.latexindent-cruft
	@echo "Finished cleaning up"

.PHONY: indent
indent: ./.latexindent.yaml ./.latexindent-cruft
	@find . -name \*.tex -exec 'latexindent' '--silent' '--overwrite' '--local=$<' '--cruft=.latexindent-cruft/' '{}' ';'
	@echo "Finished reindenting"

./.latexindent-cruft:
	@mkdir -p $@

./.latexrun:
	@echo "Unable to find .latexrun in the current directory."
	@echo "Downloading it!"
	@wget https://raw.githubusercontent.com/Nadrieril/latexrun/master/latexrun -O $@

./changebarmodified.sty:
	@echo "Unable to find $@"
	@echo "Downloading it!"
	@wget https://raw.githubusercontent.com/jaybosamiya/latex-paper-template/master/changebarmodified.sty -O $@

./.latexindent.yaml:
	@echo "Unable to find $@"
	@echo "Downloading it!"
	@wget https://raw.githubusercontent.com/jaybosamiya/latex-paper-template/master/.latexindent.yaml -O $@

.PHONY: update-makefile
update-makefile:
	@echo "Updating the current Makefile in-place"
	@wget --quiet --unlink https://raw.githubusercontent.com/jaybosamiya/latex-paper-template/master/Makefile -O Makefile

ifneq ($(MAIN_TARGET),)
.PHONY: diff-%
diff-%: FORCE ./.latexrun ./changebarmodified.sty
	@echo "Generating diff against revision $*"
	@latexdiff-vc --git -r $* --flatten --exclude-textcmd="author" -t CCHANGEBAR --force $(MAIN_TARGET:.tex=).tex >/dev/null
	@echo "Modern LaTeX has issues with the very old changebar package when floats get involved. Making sure to use the local version of changebar."
	@$(SED) -i 's/{changebar}/{changebarmodified}/' $(MAIN_TARGET:.tex=)-diff$*.tex
	@echo "Generated $(MAIN_TARGET:.tex=)-diff$*.tex. Attempting to compile it."
	@$(LATEXRUN) $(MAIN_TARGET:.tex=)-diff$*.tex
	@echo "Generated $(MAIN_TARGET:.tex=)-diff$*.pdf."

ifneq ($(DIFF_REVISIONS),)
diff: FORCE ./.latexrun
	@$(MAKE) $(patsubst %,diff-%,$(DIFF_REVISIONS))
endif
endif

.PHONY: watch
watch: all
	@echo "Finished initial (re)build. Now watching."
	fswatch --one-per-batch $(shell find . -name \*.tex) $(shell find . -name \*.bib) | xargs -n1 -I'{}' make all

# Force all intermediate files to be saved even in chains of implicits
.SECONDARY:

